Sampling Rates for $\ell^1$-Synthesis

This work investigates the problem of signal recovery from undersampled noisy sub-Gaussian measurements under the assumption of a synthesis-based sparsity model. Solving the $\ell^1$-synthesis basis pursuit allows for a simultaneous estimation of a coefficient representation as well as the sought-for signal. However, due to linear dependencies within redundant dictionary atoms it might be impossible to identify a specific representation vector, although the actual signal is still successfully recovered. The present manuscript studies both estimation problems from a non-uniform, signal-dependent perspective. By utilizing recent results on the convex geometry of linear inverse problems, the sampling rates describing the phase transitions of each formulation are identified. In both cases, they are given by the conic Gaussian mean width of an $\ell^1$-descent cone that is linearly transformed by the dictionary. In general, this expression does not allow a simple calculation by following the polarity-based approach commonly found in the literature. Hence, two upper bounds involving the sparsity of coefficient representations are provided: The first one is based on a local condition number and the second one on a geometric analysis that makes use of the thinness of high-dimensional polyhedral cones with not too many generators. It is furthermore revealed that both recovery problems can differ dramatically with respect to robustness to measurement noise -- a fact that seems to have gone unnoticed in most of the related literature. All insights are carefully undermined by numerical simulations.

==> content/illustrations.tex <==
\section{Numerical experiments}
\label{sec:num_exp}

\subsection{Sampling rates for coefficient recovery}
\label{sec:num_coef}

The purpose of this section is to illustrate the main aspects of the results on coefficient recovery by conducting numerical simulations. In particular, we want to shed light on the following claims:

\begin{enumerate}[(i)]
 \item The convex program \coefNoisefree{} obeys a sharp \emph{phase transition} in the number of measurements $m$: recovery of a coefficient vector $\gtz$ fails if $m$ is below a certain threshold and succeeds with overwhelming probability once a small transition region is surpassed; 
 
 \item $\cmw[2]{\Dict \cdot \ds{\Onenorm;\gtz}}$ accurately describes the sampling rate of \coefNoisefree{}; cf.~Theorem~\ref{thm:coeff};
 
  \item In contrast, $\cmw[2]{\ds{\Onenorm;\gtz}}$ does not describe the sampling rate of \coefNoisefree{}, in general; 
 
 \item For two minimal $\ell^1$-representations $\vec{z_1},\vec{z_2}$ with the same sparsity, but with different supports, the quantities $\cmw[2]{\Dict \cdot \ds{\Onenorm;\vec{z_1}}}$  and $\cmw[2]{\Dict \cdot \ds{\Onenorm;\vec{z_2}}}$ might differ significantly, while $\cmw[2]{\ds{\Onenorm;\vec{z_1}}} = \cmw[2]{\ds{\Onenorm;\vec{z_2}}}$. Hence, sparsity alone does not appear to be a good proxy for the sampling complexity of \coefNoisefree{}. A refined understanding of coefficient recovery requires a theory that is \emph{non-uniform} across the class of all $s$-sparse signals. 
 
 \item The local condition number $\condi{\Dict}{\gtz}$ might explode, which often renders a condition bound as in Equation~\eqref{eq:condbound} unreasonable;

\end{enumerate}
Lastly, regarding the assumptions and error bounds of Theorem~\ref{thm:coeff}, we also wish to clarify on: 

\begin{enumerate}
  \item[(vi)] Whether $\lmin{\Dict}{\dc{\Onenorm;\gtz}} \neq 0$, i.e., whether coefficient recovery is possible, is again a property that is non-uniform in the sparsity of $\gtz$;

 \item[(vii)] The value of $\lmin{\Dict}{\dc{\Onenorm;\gtz}}$ influences the robustness to noise of~\eqref{eq:coef}. 
\end{enumerate}
However, we postpone a discussion of the latter aspects to Section~\ref{sec:sampling_sig}, as it will be carried out by a comparison with signal recovery via solving~\eqref{eq:sig}.


In order to visualize the previous points, we will create \emph{phase transition plots} by running Experiment~\ref{exp:coef} for different dictionaries and signal combinations. For general design principles and more details on our simulations we refer the interested reader to Appendix~\ref{sec:num_details}. To the best of our knowledge, all other compressed sensing results on coefficient recovery with redundant dictionaries describe the sampling rate as an asymptotic upper bound.  Hence, these results are not compatible with the experiments in this section and will not be further considered. 

\begin{experiment}[Phase transition for a fixed coefficient vector]\leavevmode
\label{exp:coef}
\vspace{-.25\baselineskip}\hrule\vspace{.5\baselineskip}

\myhangindent{Input: \ }
\expkwd{Input:} Dictionary $\Dict \in \R^{n \times d}$, coefficient vector $\gtz \in \R^d$.

\vspace{.5\baselineskip}
\expkwd{Compute:} Repeat the following procedure $100$ times for every $m =1,2,\dots,n$:
\begin{expstep}
	 \item 
		Draw a standard i.i.d.\ Gaussian random matrix $\Meas \in \R^{m\times n}$ and determine the measurement vector $\y = \Meas\Dict\gtz$.
	\item 
		Solve the program \coefNoisefree{} to obtain an estimator $\solz \in \R^d$. 
	\item
		Compute and store the recovery error $\norm{\gtz - \solz}_2$. Declare success if $\norm{\gtz - \solz}_2 < 10^{-5}$.
\end{expstep}
\end{experiment}

Our first two examples are based on a \emph{redundant Haar wavelet frame}, which can be seen as a typical representation system in the field of applied harmonic analysis, see~\cite{mallat09} for more details on wavelets and Section 3.1 in~\cite{genzel2017} for a short discussion in the context of compressed sensing. As a back-end for defining the wavelet transform, we are using the \texttt{Matlab} software package \texttt{spot}~\cite{spot}, which is in turn based on the \texttt{Rice Wavelet Toolbox}~\cite{rwt}. We set the ambient dimension to $n=256$ and consider a Haar system with $3$ decomposition levels and normalized atoms. The resulting dictionary is denoted by $\Dictw \in \R^{256 \times 1024}$. 
The first coefficient vector $\vec{z_1} \in \R^{1024}$ is obtained by selecting a random support set of cardinality $s=16$, together with random coefficients; see Subplot~\ref{fig:coef:wave:3} for a visualization of $\vec{z_1}$ and Subplot~\ref{fig:coef:wave:2} for the resulting signal $\vec{x_1} = \Dict \vec{z_1}$. The second coefficient vector $\vec{z_2}$ is created by defining two contiguous blocks of non-zero coefficients in the low frequency part, again with $s=16$; see Subplot~\ref{fig:coef:wave:6} for a plot of $\vec{z_2}$ and Subplot~\ref{fig:coef:wave:5} for the resulting signal $\vec{x_2} = \Dict \vec{z_2}$. For each signal we run Experiment~\ref{exp:coef} and report the empirical success rate in the Subplots \ref{fig:coef:wave:1}, \ref{fig:coef:wave:4}, respectively.

In the third example, the dictionary is chosen as a \emph{Gaussian random matrix}, which is a typical benchmark system for compressed sensing with redundant frames, see~for instance \cite{genzel2017,kabanava2015,chen2014}. Also in this case, we set $n= 256$, but we choose $d=512$. The resulting dictionary is denoted by $\Dict_{\texttt{rand}} \in \R^{256\times 512}$. The coefficient vector $\vec{z_3}$ is  defined in the same manner as $\gtz$ above, where we again have $\norm{\vec{z_3}}_0=16$. The resulting signal $\vec{x_3}$ is shown in Subplot~\ref{fig:coef:wave:8} and the empirical success rate in Subplot~\ref{fig:coef:wave:7}.       

Our fourth and last dictionary is inspired by \emph{super-resolution}; see for instance~\cite{candes2012}. We again set $n=256$ and set the dictionary $\Dict_{\texttt{super}} \in \R^{256 \times 256}$ as a convolution with a discrete Gaussian function of large variance. This example can therefore be considered as a finely discretized super resolution problem. The coefficient vector $\vec{z_4}$ is then chosen as a sparse vector with $z_{4,128} = 1$ and $z_{4,129} = -1$, see Subplot~\ref{fig:coef:wave:12}. Hence, in the signal $\vec{x_4}$, the two neighboring peaks almost cancel out and result in the low amplitude signal shown in Subplot~\ref{fig:coef:wave:11}. Finally, the empirical success rate is depicted in Subplot~\ref{fig:coef:wave:10}.  
Note that for each example we have verified the necessary condition $\lmin{\Dict}{\dc{\Onenorm,\vec{z_i}}} > 0$ heuristically by checking if $\Zlset = \left\{ \vec{z_i} \right\}$ for each $i=1,\dots,4$.  


Let us now return to the previously listed Claims (i)-(v) by inspecting the empirical success rates of Figure~\ref{fig:coef:wave} and comparing them with the estimates of $\cmw[2]{\Dict \cdot \ds{\Onenorm;\vec{z_i}}}$ and $\cmw[2]{\ds{\Onenorm;\vec{z_i}}}$:
It is clear that all simulations obey a sharp phase transition in $m$. This observation could have been anticipated, given for instance the works~\cite{amelunxen2014edge,tropp2014convex}. However, note that the product structure of the matrix $\Meas\Dict$ in \coefNoisefree{} does not allow for a direct application of these results. 
Considering Remark~\ref{rem:coef}, claim (ii) is also well reflected in all experiments. Regarding Claim (iii), we first observe that $\cmw[2]{\Dict \cdot \ds{\Onenorm;\vec{z_i}}}$ and  $\cmw[2]{\ds{\Onenorm;\vec{z_i}}}$ are really close (albeit still different) in the Subplots~\ref{fig:coef:wave:1} and~\ref{fig:coef:wave:6}. However, in the remaining two examples, $\cmw[2]{\ds{\Onenorm;\vec{z_i}}}$ significantly departs from the actual location of the phase transition.  Note in particular, that $\cmw[2]{\Dict \cdot \ds{\Onenorm;\vec{z_4}}} \gg \cmw[2]{\ds{\Onenorm;\vec{z_4}}}$ while $\cmw[2]{\Dict \cdot \ds{\Onenorm;\vec{z_2}}} \ll \cmw[2]{\ds{\Onenorm;\vec{z_2}}}$. By comparing the Subplots~\ref{fig:coef:wave:1} and \ref{fig:coef:wave:4} we can verify claim (iv). Although the support sets of $\vec{z_1}$ and $\vec{z_2}$ are different, the sparsity is the same and therefore we observe that $\cmw[2]{\ds{\Onenorm;\vec{z_1}}} = \cmw[2]{\ds{\Onenorm;\vec{z_2}}}$ up to small numerical errors. However, since $\cmw[2]{\Dict \cdot \ds{\Onenorm;\vec{z_1}}}$ and $\cmw[2]{\Dict \cdot \ds{\Onenorm;\vec{z_2}}}$ are far apart, it turns out that coefficient vectors with the same sparsity may indeed result in different sampling rates for \coefNoisefree{}. This stresses once again the importance of establishing non-uniform results. Lastly, regarding Claim (v), we have reported upper bounds for $\lmin{\Dict}{\dc{\Onenorm,\vec{z_i}}}$ in Figure~\ref{fig:coef:wave}. Since the norms of each dictionary are well controlled, the latter quantities are responsible for unreasonably large values of $\condi{\Dict}{\vec{z_i}}$. This shows that condition number estimates as in Equation \eqref{eq:condbound} are too pessimistic in many situations. 

\begin{figure}[!t]
	\centering
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/coeff/wave/pt_1d_wave.png}
		\caption{}
		\label{fig:coef:wave:1}
	\end{subfigure}%
	\qquad
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/coeff/wave/signal.png}
		\caption{}
		\label{fig:coef:wave:2}
	\end{subfigure}%	
	\qquad
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/coeff/wave/coeff.png}
		\caption{}
		\label{fig:coef:wave:3}
	\end{subfigure}%
	\vspace{.5\baselineskip}
		\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/coeff/wave/pt_1d_wave_constSig.png}
		\caption{}
		\label{fig:coef:wave:4}
	\end{subfigure}%
	\qquad
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/coeff/wave/signal_constSig.png}
		\caption{}
		\label{fig:coef:wave:5}
	\end{subfigure}%	
	\qquad
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/coeff/wave/coeff_constSig.png}
		\caption{}
		\label{fig:coef:wave:6}
	\end{subfigure}%
	\vspace{.5\baselineskip}
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/coeff/rand/pt_1d_rand.png}
		\caption{}
		\label{fig:coef:wave:7}
	\end{subfigure}%
	\qquad
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/coeff/rand/signal.png}
		\caption{}
		\label{fig:coef:wave:8}
	\end{subfigure}%	
	\qquad
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/coeff/rand/coeff.png}
		\caption{}
		\label{fig:coef:wave:9}
	\end{subfigure}%
	\vspace{.5\baselineskip}
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/coeff/super/pt_1d_super.png}
		\caption{}
		\label{fig:coef:wave:10}
	\end{subfigure}%
	\qquad
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/coeff/super/signal.png}
		\caption{}
		\label{fig:coef:wave:11}
	\end{subfigure}%	
	\qquad
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/coeff/super/coeff.png}
		\caption{}
		\label{fig:coef:wave:12}
	\end{subfigure}%
	\caption{Phase transitions of coefficient recovery by solving \coefNoisefree{} for different coefficient and dictionary setups. Empirical success rates and other key figures are reported in the first column, where we have used the short hand notation $\mathcal{D} =\ds{\Onenorm,\vec{z_i}}$. The coefficient vectors $\vec{z_i}$ that were used in each experiment are shown in the third column. The associated signal vectors $\vec{x_i} = \Dict \vec{z_i}$ are displayed in the second column. The first two rows are relying on a redundant Haar wavelet frame, the third row is based on a Gaussian random matrix and the last row is using a dictionary inspired by super-resolution. }
	\label{fig:coef:wave}
\end{figure}

Let us conclude this section by summarizing our findings regarding coefficient recovery by:

\begin{highlight}
 The required number of sub-Gaussian measurements for robust recovery of a coefficient vector $\gtz$ via solving \eqref{eq:coef} -- implying thereby also recovery of the signal $\gt = \Dict \gtz$ -- is determined by the conic mean width $\cmw[2]{\Dict \cdot \ds{\Onenorm;\gtz}}$.
    It is possible to formulate an (non-tight) upper bound involving the sparsity $s = \# \supp (\gtz)$ and a local condition number $\condi{\Dict}{\gtz}$ of $\Dict$ at $\gtz$. The latter factor is thereby intimately related to the necessary assumption that $\gtz$ is the unique $\ell^1$-representation of $\gt$.
\end{highlight}

\subsection{Sampling rates for signal recovery}
\label{sec:sampling_sig}
Here, we wish to shed light on the following claims regarding the sampling rate of signal recovery:

\begin{enumerate}[(i)] 

  \item The convex program \sigNoisefree{} obeys a sharp \emph{phase transition} in the number of measurements, c.f.~Claim (i) in Section~\ref{sec:num_coef}. This phenomenon occurs although a corresponding reconstruction of coefficients via \coefNoisefree{} might not be successful;

  \item For a $\zl \in \Zlset$, the conic mean width $\cmw[2]{\Dict \cdot \ds{\Onenorm;\zl}}$ accurately describes the sampling rate for recovering $\gt$ via solving \sigNoisefree{}, see~Theorem~\ref{thm:sig};
 
  \item In contrast, for an arbitrary sparse representation $\gtz \in \R^d \setminus \Zlset$  of $\gt$ in  $\Dict$, the mean width $\cmw[2]{\Dict \cdot \ds{\Onenorm;\gtz}}$ does not describe the sampling rate of \sigNoisefree{}, in general. Hence, sparsity alone is typically not a good proxy for the sample complexity of signal recovery.  
  %A refined understanding requires a theory that is \emph{non-uniform} across the class of all $s$-sparse signals; c.f.~Claim (iv) in Section~\ref{sec:num_coef}. 
\end{enumerate}

As already carried out in Section~\ref{sec:num_coef}, in order to visualize the previous claims, we will create \emph{phase transition plots} by running Experiment~\ref{exp:coef} for different dictionaries and signal combinations; see also Appendix~\ref{sec:num_details} for general design principles. Note that in these experiments, we additionally compute and store the signal recovery error $\norm{\gt - \sol}_2 = \norm{\Dict \cdot \gtz - \Dict \cdot \solz}_2$ in the third step of the experiment. Recovery is declared successful if $\norm{\gt - \sol}_2 < 10^{-5}$. To the best of our knowledge, all other compressed sensing results on signal recovery with redundant dictionaries describe the sampling rate as an asymptotic upper bound.  Hence, these results, as well as Theorem~\ref{thm:sig}, are not compatible with the experiments in this section and will not be further considered. 

Our first two examples are based on the same Haar wavelet system with 3 decomposition levels that is used in Section~\ref{sec:num_coef}, i.e., we choose $n= 256, d = 1024$ and denote the resulting dictionary by $\Dictw \in \R^{256\times 1024}$. The first signal is constructed by defining a coefficient vector $\vec{z_1} \in \R^{1024}$ with a random support set of cardinality $s=35$ and random coefficients; see Subplot~\ref{fig:sig:wave:10} for a visualization of $\vec{z_1}$ and Subplot~\ref{fig:coef:wave:2} for the resulting signal $\vec{x_1} = \Dictw \cdot \vec{z_1}$. In order to apply the result of Theorem~\ref{thm:sig}, we compute a minimal $\ell^1$-representation $\zl^1 \in \Zlset$ of $\vec{x_1}$; see Subplot~\ref{fig:sig:wave:7}. 
The second coefficient vector $\vec{z_2}$ is created by defining two contiguous blocks of non-zero coefficients in a lower frequency decomposition scale, again with $s=35$; see Subplot~\ref{fig:sig:wave:11} for a plot of $\vec{z_2}$ and Subplot~\ref{fig:sig:wave:5} for the resulting signal $\vec{x_2} = \Dictw  \cdot \vec{z_2}$. The corresponding minimal $\ell^1$-representation $\zl^2 \in \Zlset$ of $\vec{x_2}$ is shown in Subplot~\ref{fig:sig:wave:8}. 

Finally, for the third setup we are choosing a simple example in 2D. In order to keep the computational burden manageable, we restrict ourselves to a $28 \times 28$-dimensional digit from the MNIST data set~\cite{mnist}, i.e., the vectorized image is of size $n=28^2 = 784$. As a sparsifying system we utilize a dictionary that is based on the \emph{2D discrete cosine transform} (2D-DCT). It makes use of \texttt{Matlab}'s standard 2D-DCT transform as convolution filters on $3 \times 3$ patches. The resulting operator is denoted by $\Dict \in \R^{n \times 9\cdot n}$, i.e., $d = 9\cdot n$. Note that such a convolution sparsity model is frequently used in the literature, in particular also with learned filters, e.g., see \emph{convolutional sparse coding} in \cite{bristow2013}. Although the 2D-DCT filters might not be a perfect match for MNIST digits, we consider them as a classical representative that is well suited to demonstrate the predictive power of our results. In order to construct a suitable sparse representation $\vec{z_3}\in\R^d$ of an arbitrarily picked digit in the database, we make use of the \emph{orthogonal matching pursuit} algorithm~\cite{omp1993}; see Subplot~\ref{fig:sig:wave:12} for a visualization of $\vec{z_3}$. The resulting digit $\vec{x_3} = \Dict \cdot \vec{z_3}$ is displayed in Figure~\ref{fig:sig:wave:6}. A minimal $\ell^1$-representation $\zl^3$, which is needed to apply Theorem~\ref{thm:sig}, is shown in Subplot~\ref{fig:sig:wave:9}.     

Let us now return to the previously listed Claims (i)-(iii) by inspecting the empirical success rates in Figure~\ref{fig:sig:wave} and comparing them with the estimates of the quantities $\cmw[2]{\Dict \cdot \ds{\Onenorm;\zl^i}}$ and $\cmw[2]{\Dict \cdot \ds{\Onenorm;\vec{z_i}}}$:
It is clear that all three simulations obey a sharp phase transition in $m$ with respect to signal recovery. Due to the gauge-based reformulation~\eqref{eq:gauge} of \sigNoisefree{} this observation is predicted by the works~\cite{amelunxen2014edge,tropp2014convex}. However, note that in none of the examples, recovery of a coefficient representation via solving \coefNoisefree{} is possible; not even for $m=n$. The second claim is a direct consequence of Theorem~\ref{thm:sig} and is well reflected in all three cases since $\cmw[2]{\Dict \cdot \ds{\Onenorm;\zl^i}}$ matches precisely the 50\% recovery rate. Regarding Claim (iii), we observe in all simulations, that $\cmw[2]{\Dict \cdot \ds{\Onenorm;\vec{z_i}}} \approx n$, which shows that this quantity does not allow to characterize the sampling rate for perfect recovery. In that regard, also note that $\norm{\vec{z_1}}_0 = 35 = \norm{\vec{z_2}}_0$, however, the locations of the phase transitions deviate considerably. Similarly, although $\norm{\zl^1}_0 < \norm{\zl^2}_0$, we have that $\cmw[2]{\Dict \cdot \ds{\Onenorm;\zl^1}} > \cmw[2]{\Dict \cdot \ds{\Onenorm;\zl^2}}$. This observation is yet another indication that, in general, $\ell^0$-sparsity is not a good proxy for the sampling rate.
 


We conclude this section by discussing the phase transition plots shown in Figure~\ref{fig:sig:pt_2}. In particular, these results also give numerical indication for Claim (vi) in Section~\ref{sec:num_coef}. Up to now, we have only considered one specific signal at a time. However, it is also of interest to assess the quality of our results if the ``complexity'' of the underlying signals is varied. In the classical situation of $\Dict$ being an ONB, the location of the phase transition is entirely determined by the sparsity of the underlying signal. Hence, it is a natural choice to create phase transitions over the sparsity, as it is for instance done in \cite{amelunxen2014edge}. Recalling Claim (iii) in this section and Claim (iv) in Section~\ref{sec:num_coef}, it might appear odd to also choose sparsity as a measure for complexity in the case of a redundant dictionary. However, as the result of Figure~\ref{fig:sig:pt_2} shows, if the support is chosen uniformly at random, sparsity is still a somewhat reasonable proxy for the sampling rate.  Indeed, these plots are created by running Experiment~\ref{exp:pt} with $\Dict = \Dictw \in \R^{256\times 1024}$, maximal sparsity $s_0 = 125$ and displaying the empirical success rates of coefficient and signal recovery, respectively. Additionally the dotted line shows the averaged conic mean width values $\cmw[2]{\Dict \cdot \ds{\Onenorm;\zl}}$.  

\begin{experiment}[Phase transition of Figure~\ref{fig:sig:pt_2}]\leavevmode
\label{exp:pt}
\vspace{-.25\baselineskip}\hrule\vspace{.5\baselineskip}

\myhangindent{Input: \ }
\expkwd{Input:} Dictionary $\Dict \in \R^{n \times d}$, maximal sparsity $s_0 \in [n]$. 

\vspace{.5\baselineskip}
\expkwd{Compute:} Repeat the following procedure $200$ times for each $s \in \{1,\dots,s_0\}$:
\begin{expstep}
	\item 
	 Select a set $S \subset [n]$ uniformly at random with $\# S = s$. Then draw a standard Gaussian random vector $\vec{c} \in \R^s$ and define $\gtz$ by setting $(\gtz)_S = \vec{c}$ and $(\gtz)_{\setcompl{S}} = \vec{0}$. 
	\item 
	 Define the signal $\gt = \Dict \cdot \gtz$ and compute a minimal $\ell^1$-representation $\zl\in\Zlset$ of $\gt$. Compute the conic mean width $\cmw[2]{\Dict \cdot \ds{\Onenorm;\zl}}$. 
	\item 
     Run Experiment~\ref{exp:coef} with $\Dict$ and $\zl$ as input, where the number of repetitions is lowered to 5. Thereby, in the third step, coefficient/signal recovery is declared successful if $\norm{\gtz -  \solz}_2 < 10^{-5}$ or if $ \norm{\Dict \cdot \gtz - \sol}_2 = \norm{\gt - \Dict \cdot \solz}_2 < 10^{-5}$, respectively.
\end{expstep}
\end{experiment}

First note, that the averaged values of the conic mean width perfectly match the center of the phase transition in Subplot~\ref{fig:sig:pt_2:2}, as it is predicted by Theorem~\ref{thm:sig}. However, also observe that for sparsity values between $s \approx 20$ and $s\approx 80$ the transition region is spread out in the vertical direction, c.f.~\cite{amelunxen2014edge}. As mentioned above, this can be related to Claim (iii): given that sparsity alone is not a good proxy for the sample complexity of \sigNoisefree{}, averaging over different instances with the same sparsity, necessarily results in a smeared out transition area.  Nevertheless, if the coefficients are chosen at random as in Experiment~\ref{exp:pt}, it is still possible to observe a relatively sharp transition in the number of required measurements. 


Regarding the phase transition in Subplot~\ref{fig:sig:pt_2:1}, we observe that for sparsity values $\norm{\gtz}_0\geq50$, recovery of coefficients appears to be impossible. On the other hand, for very small sparsity (i.e., $\norm{\gtz}_0\leq 5$), signal and coefficient recovery seem to be equivalent. The interval in between constitutes a transition region, in which coefficient recovery becomes gradually less likely. We suspect that with more repetitions in Experiment~\ref{exp:pt}, the empirical success rates on this interval would eventually also smooth out. The existence of such a relatively wide transition area gives evidence for Claim (vi) in Section~\ref{sec:num_coef}: sparsity alone does not determine whether coefficient recovery is possible or not.%\footnote{Note that Claim (vi) would actually prescribe to consider $\norm{\zl}_0$ instead of $\norm{\gtz}_0$. However, there is a strong correlation between booth quantities, which still allows us to draw the conclusion above; see Figure~\ref{fig:corr} in the Appendix.}.
 As predicted by Theorem~\ref{thm:coeff}, if coefficient recovery is possible, the location of the phase transition is also determined by $\cmw[2]{\Dict \cdot \ds{\Onenorm;\zl}}$, c.f.~Subplot~\ref{fig:sig:pt_2:2}. However, if $\lmin{\Dict}{\dc{\Onenorm,\zl}} = 0$, recovery of coefficients is impossible for any $m$; this explains the ``vertical stripes'' above the dotted line. Overall, comparing the areas above the mean width allows to obtain a qualitative visualization of the relationship of coefficient and signal recovery under the random model of Experiment~\ref{exp:pt}.         


\begin{figure}[!t]
	\centering
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/signal/wave/pt_1d_wave.png}
		\caption{}
		\label{fig:sig:wave:1}
	\end{subfigure}%
	\qquad
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/signal/wave/pt_1d_wave_constSig.png}
		\caption{}
		\label{fig:sig:wave:2}
	\end{subfigure}%	
	\qquad
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/signal/dct/pt_1d_dct_MNIST.png}
		\caption{}
		\label{fig:sig:wave:3}
	\end{subfigure}%
	\vspace{.5\baselineskip}
		\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/signal/wave/signal.png}
		\caption{}
		\label{fig:sig:wave:4}
	\end{subfigure}%
	\qquad
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/signal/wave/signal_const.png}
		\caption{}
		\label{fig:sig:wave:5}
	\end{subfigure}%	
	\qquad
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/signal/dct/signal.png}
		\caption{}
		\label{fig:sig:wave:6}
	\end{subfigure}%
	\vspace{.5\baselineskip}
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/signal/wave/coeff.png}
		\caption{}
		\label{fig:sig:wave:7}
	\end{subfigure}%
	\qquad
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/signal/wave/coeff_const.png}
		\caption{}
		\label{fig:sig:wave:8}
	\end{subfigure}%	
	\qquad
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/signal/dct/coeff.png}
		\caption{}
		\label{fig:sig:wave:9}
	\end{subfigure}%
	\vspace{.5\baselineskip}
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/signal/wave/coeff_0.png}
		\caption{}
		\label{fig:sig:wave:10}
	\end{subfigure}%
	\qquad
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/signal/wave/coeff_const_0.png}
		\caption{}
		\label{fig:sig:wave:11}
	\end{subfigure}%	
	\qquad
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/signal/dct/coeff_0.png}
		\caption{}
		\label{fig:sig:wave:12}
	\end{subfigure}%
	\caption{Phase transitions of signal recovery by solving \sigNoisefree{} for different signal and dictionary setups. Empirical success rates and other key figures are reported in the first row, where we have used the short hand notation $\mathcal{D}_1 = \ds{\Onenorm,\zl^i}$ and $\mathcal{D}_0 = \ds{\Onenorm,\vec{z_i}}$. The signals $\vec{x_i}$ that were used in each experiment are shown in the second row. The associated minimal $\ell^1$-representations $\zl^i$ are displayed in the third row and the original, defining coefficient representations $\vec{z_i}$ are shown in the fourth row. The first two columns are relying on a redundant Haar wavelet frame and the third column is based on the 2D-DCT. Note that in all three examples, coefficient recovery is not possible since $\lmin{\Dict}{\dc{\Onenorm,\zl^i}} = 0$.}
	\label{fig:sig:wave}
\end{figure}



\subsection{Robustness to Noise}
\label{sec:robustness_noise}

The purpose of this last numerical simulation is to analyze coefficient and signal recovery with respect to robustness to measurement noise. In particular, we want to shed light on the following claims:

\begin{enumerate}[(i)] 

  \item If the number of measurements exceeds the sampling rate in Theorem~\ref{thm:sig}, signal recovery via solving the Program~\eqref{eq:sig} is robust to measurement noise. This phenomenon holds true without any further assumptions. 
  
  \item If $\gtz$ is the unique minimal $\ell^1$-representation of $\gt$ (i.e., if $\lmin{\Dict}{\dc{\Onenorm,\gtz}} > 0$) and if the number of measurements exceeds the sampling rate in Theorem~\ref{thm:coeff}, it is possible to robustly recovery $\gtz$. However, in contrast to signal recovery, the robustness is heavily influenced by the ``stability'' of the minimal $\ell^1$-representation of $\gtz$ in $\Dict$, i.e., by the value of $\lmin{\Dict}{\dc{\Onenorm,\gtz}}$ in the error bound~\eqref{eq:rec_coef}.
  
  \item Hence, if $\lmin{\Dict}{\dc{\Onenorm,\gtz}} > 0$, it is possible that the signal $\gt$ is more robustly recovered than its coefficients $\gtz$, or vice versa (depending on $\lmin{\Dict}{\dc{\Onenorm,\gtz}}$). 
  
\end{enumerate}
  


In order to visualize the previous claims, we run Experiment~\ref{exp:robust} for different setups. First, we choose the same dictionary and signal combination as in Section~\ref{sec:num_coef} and restrict the noise level to $H = \left\{0,0.05,0.1,0.15,\dots,1 \right\}$. Furthermore, we consider the 1D examples of Section~\ref{sec:sampling_sig}, together with the noise range $H = \left\{0,0.005,0.01,\dots,0.1 \right\}$. Recall that the difference of these two setups is that $\lmin{\Dict}{\dc{\Onenorm,\zl}} > 0$ in the first case and that $\lmin{\Dict}{\dc{\Onenorm,\zl}} = 0$ in the second, where $\zl \in \Zlset$. In all experiments, we roughly pick the number of measurements as $m \approx \cmw[2]{\Dict \cdot \ds{\Onenorm;\zl}} +40$ to ensure that the Theorem~\ref{thm:coeff} or Theorem~\ref{thm:sig} is applicable. The averaged coefficient and signal recovery errors are displayed in Figure~\ref{fig:noise}, together with the upper bound on the signal error, see Equation~\eqref{eq:rec_sig1}. Note that it is not possible to show the corresponding error bound for coefficient recovery. In the first set of examples, we don't have access to $\lmin{\Dict}{\dc{\Onenorm,\zl}}$ and in the last two cases, $\lmin{\Dict}{\dc{\Onenorm,\zl}} = 0$ and thus, Theorem~\ref{thm:coeff} is not applicable. Nevertheless, it is possible to obtain an upper bound for the latter quantity, as outlined in the Appendix~\ref{sec:num_details}. If $\Dict = \Dict_{\texttt{rand}}$, it is possible to use the result on minimum conic singular values of Gaussian matrices to get a lower bound with high probability, see for instance \cite[Prop. 3.3]{tropp2014convex}.

\begin{experiment}[Robustness to Measurement Noise]\leavevmode
\label{exp:robust}
\vspace{-.25\baselineskip}\hrule\vspace{.5\baselineskip}

\myhangindent{Input: \ }
\expkwd{Input:} Dictionary $\Dict \in \R^{n \times d}$, number of measurements $m$, minimal $\ell^1$-representation $\zl$ of the signal $\gt \in \R^n$, range of noise levels $H$.

\vspace{.5\baselineskip}
\expkwd{Compute:} Repeat the following procedure $100$ times for every $\noiseparam \in H$:
\begin{expstep}
	 \item 
		Draw a standard i.i.d.\ Gaussian random matrix $\Meas \in \R^{m\times n}$ and determine the noisy measurement vector $\y = \Meas\gt + \noiseparam \cdot \noise$, where $\norm{\noise}_2 = 1$.
	\item 
		Solve the program \eqref{eq:coef} to obtain an estimator $\solz \in \R^d$. 
	\item
		Compute and store the recovery errors $\norm{\zl - \solz}_2$ and $\norm{\gt - \sol}_2 = \norm{\Dict \cdot \zl - \Dict \cdot \solz}_2$.
\end{expstep}
\end{experiment}

Returning to the claims listed above, the first one is clearly reflected in all results of Figure~\ref{fig:noise}. Observe thereby that the actual error $\norm{\gt - \sol}$ lies below its theoretical upper bound of Equation~\eqref{eq:rec_sig1}. However, this is not surprising, since the measurement error $\noise$ used in Experiment~\ref{exp:robust}, is most likely not the worst possible  instance of adversarial noise.  Also Claim (ii) can be easily verified by inspecting the examples shown in the Subplots~\ref{fig:noise:1}-\ref{fig:noise:4}. However, note that the quantity  $\lmin{\Dict_{\texttt{super}}}{\dc{\Onenorm,\zl}}$ is minuscule. Hence, even for a small amount of noise the error of Equation~\eqref{eq:rec_coef} explodes. For $\noiseparam>0.1$ the error stays roughly constant since the solution $\solz$ of \eqref{eq:coef} is always close to $\vec{0}$. As it can be seen from the Examples shown in Subplot~\ref{fig:noise:5} and Subplot~\ref{fig:noise:6}, $\lmin{\Dict}{\dc{\Onenorm,\zl}} > 0$ is a necessary condition for robust recovery of $\zl$, however, it does not affect robust recovery of the signal $\gt$. 
Lastly, by comparing coefficient and signal recovery in the first four cases, we justify Claim (iii). Indeed, if $\lmin{\Dict}{\dc{\Onenorm,\zl}}  \ll 1$, coefficient recovery is less robust than signal recovery, see Subplots~\ref{fig:noise:1}, \ref{fig:noise:2} and \ref{fig:noise:4}. However, if $\lmin{\Dict}{\dc{\Onenorm,\zl}}  \gg 1$, the contrary holds true, see Subplot~\ref{fig:noise:3}. 


\begin{figure}
	\centering
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/coeff/wave/noise.png}
		\caption{}
		\label{fig:noise:1}
	\end{subfigure}%
	\qquad
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/coeff/wave/noise_constSig.png}
		\caption{}
		\label{fig:noise:2}
	\end{subfigure}%	
	\qquad
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/coeff/rand/noise.png}
		\caption{}
		\label{fig:noise:3}
	\end{subfigure}
    \vspace{.5\baselineskip}
    \begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/coeff/super/noise.png}
		\caption{}
		\label{fig:noise:4}
	\end{subfigure}%
	\qquad
    \begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/signal/wave/noise.png}
		\caption{}
		\label{fig:noise:5}
	\end{subfigure}%
	\qquad
	\begin{subfigure}[t]{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/signal/wave/noise_constSig.png}
		\caption{}
		\label{fig:noise:6}
	\end{subfigure}%
	\caption{Robust coefficient and signal recovery for different dictionary and coefficient/signal combinations. The first four Subplots are based on the examples for coefficient recovery in Section~\ref{sec:num_coef}, and the the last two on the  examples based on Haar wavelet in Section~\ref{sec:sampling_sig}. We have used the short hand notation $\mathcal{D} = \ds{\Onenorm,\zl}$, where $\zl \in \Zlset$.}
	\label{fig:noise}
\end{figure}





